Canonical Representations of k-Safety Hyperproperties

Hyperproperties elevate the traditional view of trace properties form sets of traces to sets of sets of traces and provide a formalism for expressing information-flow policies. For trace properties, algorithms for verification, monitoring, and synthesis are typically based on a representation of the properties as omega-automata. For hyperproperties, a similar, canonical automata-theoretic representation is, so far, missing. This is a serious obstacle for the development of algorithms, because basic constructions, such as learning algorithms, cannot be applied. In this paper, we present a canonical representation for the widely used class of regular k-safety hyperproperties, which includes important polices such as noninterference. We show that a regular k-safety hyperproperty S can be represented by a finite automaton, where each word accepted by the automaton represents a violation of S. The representation provides an automata-theoretic approach to regular k-safety hyperproperties and allows us to compare regular k-safety hyperproperties, simplify them, and learn such hyperproperties. We investigate the problem of constructing automata for regular k-safety hyperproperties in general and from formulas in HyperLTL, and provide complexity bounds for the different translations. We also present a learning algorithm for regular k-safety hyperproperties based on the L* learning algorithm for deterministic finite automata.

==> commands.tex <==
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}





\newcommand\comment[1]{}
%% Packages
\usepackage[colorlinks = true,
linkcolor = blue,
urlcolor  = blue,
citecolor = blue,
anchorcolor = blue]{hyperref}
\renewcommand\UrlFont{\color{blue}\rmfamily}
\usepackage{amsmath}
\usepackage{latexsym}
\usepackage{cleveref}
\usepackage{amssymb}
\usepackage{esvect}
\RequirePackage{color}
\usepackage{algorithmic}
\usepackage{algorithm}
%
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}

% Toogle Thesis and Paper
\usepackage{etoolbox}
\newtoggle{THESIS}
\togglefalse{THESIS}

%% Logics
\newcommand{\until}{\mathbin{\textsf{U}}}
\newcommand{\release}{\mathbin{\textsf{R}}}
\newcommand{\lnext}{\mathbin{\bigcirc}}
\DeclareMathOperator{\globally}{\raisebox{-2pt}{\scalebox{1.4}{$\Box$}}}
\DeclareMathOperator{\finally}{\raisebox{-1pt}{\scalebox{1.2}{\rotatebox[origin=c]{45}{$\Box$}}}}

%% Shortcuts
% Assitance for making notes
\newcommand\QS[1]{{\color{blue}{Question: #1}}}
\newcommand\QSS[1]{{Question solved: #1}}
\newcommand\correct[1]{{\color{green}Correct: #1}}
\newcommand{\IGNORE}[1]{}
\newcommand\TODO[1]{{\color{red} TODO: #1}}

% Special Terms in computer science
\newcommand{\PSpace}{\textsc{PSpace} }
\newcommand{\UP}{\text{UP}}


% Notations and Languages
\newcommand{\lhyper}{L$^*_{Hyper}$ }
\newcommand{\hyper}{{\mc{P}(\Sigma^{\omega})}}
\newcommand{\hyperF}{{\mc{P}(\Sigma^{*})}}
\newcommand{\bad}{\textsf{BadPref}}
\newcommand{\per}[1]{\mathfrak P(#1)}
\newcommand{\traces}{\textsf{traces}}
\newcommand{\OD}{\textsf{OD}}
\newcommand{\AP}{\text{AP}}
\newcommand{\zip}{\textsf{zip}}
\newcommand{\unzip}{\textsf{unzip}}
\newcommand{\extend}{\textsf{extend}}
\newcommand{\row}{\textsf{row}}
\newcommand{\delete}{\textsf{delete}}
\newcommand{\Prop}{\textsf{Prop}}
\newcommand{\HP}{\textsf{\textbf{HP}}}
\newcommand{\safety}{\mathbf{S}}
\newcommand{\kfa}{{k-BPA}\@\xspace}
\newcommand{\perm}{\textsf{Perm}}
\newcommand{\EQ}{\emph{EQ}}
\newcommand{\MQ}{\emph{MQ}}
\newcommand{\Reduce}{\emph{Reduce}}
\usepackage[T1]{fontenc}
\usepackage{xspace}
\newcommand{\hyperltl}{{\sc{HyperLTL}}\@\xspace}
\newcommand{\hyperctl}{{\sc{HyperCTL$^*$}}\@\xspace}
\newcommand{\ltl}{{\sc{LTL}}\@\xspace}

% standard math commands
\newcommand{\mb}[1]{{\mathbb{#1}}}
\newcommand{\mc}[1]{{\mathcal{#1}}}
\newcommand{\norm}[1]{{\left\lVert #1 \right\rVert}}
\newcommand{\abs}[1]{{\left| #1 \right|}}

% Math symbols
\newcommand{\NN}{\mathbb{N}}


% Alphabet for automata, transistion systems... :
\newcommand{\A}{\mc{A}}
\newcommand{\V}{\mc{V}}
\newcommand{\Q}{\mc{Q}}
\newcommand{\T}{\mc{T}}
\renewcommand{\S}{\mc{S}}
\newcommand{\R}{\mc{R}}
\newcommand{\TS}{\mc{TS}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\F}{\mc{F}}
\newcommand{\I}{\mc{I}}
\renewcommand{\L}{\mc{L}}
\renewcommand{\O}{\mc{O}}
\newcommand{\atomic}{\textsf{AP}}

\newcommand{\curly}[1]{\left\lbrace#1\right\rbrace}
\newcommand{\set}[1]{\curly{#1}}
\newcommand{\filter}[2]{\curly{#1 \mid #2}}
\renewcommand{\L}{\mathcal{L}}

\newcommand{\nats}{\mathbb{N}}
\newcommand{\lstar}{{L$^*$}\@\xspace}
\newcommand{\lstarhyper}{{L$^*_\mathit{Hyper}$}\@\xspace}











==> tikz/framework.tex <==
\begin{tikzpicture}
\def\x{2.5}
\def\y{5}
\def\aleft{-4.5 + \x}
\def\aright{4.5 - \x}


\draw [line width=1mm, rounded corners=3] (-4.5 - \x,-1.5) rectangle ++(5,\y) node [midway] (teacher) {};

\node [below=3 of teacher] (teacher_text) {Teacher};


\draw [line width=1mm,rounded corners=3] (\aright,-1.5) rectangle ++(1.5, \y) node [midway] (learner) {};

\node [below=3 of learner] (learner_text) {Learner};

%	\draw (-)


%%%%%%%% Queries %%%%%%%%%%%%%%%%%%%%%%%%%
% equivalenc
\path[->]
(\aright, \y - 2) edge node [label, above] {\footnotesize{$ EQ(\A)$}} (\aleft, \y - 2)
(\aleft, \y - 2.3) edge node [label, below] {yes/no + ce $\in (\Sigma^{k'})^*$} (\aright, \y - 2.3);

% membership
\path[->]
(\aright, -0.7) edge node [label, above] {\footnotesize{$MQ(x)$}} (\aleft, -0.7)
(\aleft, -1) edge node [label, below] {yes/no} (\aright, -1);


%%%%%%%% Teacher %%%%%%%%%%%%%%%%%%%%%%%%%
%% Components
\draw [line width=0.5mm] (-\x - 4, 2.2) rectangle ++ (1.5, 0.8) node [midway] (EQ) {\EQ};

\draw [line width=0.5mm] (-\x - 4, 0.6) rectangle ++ (1.5, 0.8) node [midway] (RE) {\Reduce};

\draw [line width=0.5mm] (-\x - 4, -1) rectangle ++ (1.5, 0.8) node [midway] (MQ) {\MQ};

%% Lines
%%% EQ
\draw [->, >=stealth, thick,shorten >=2pt] plot [smooth] coordinates {(\aleft, \y-2) (\aleft -1, \y - 2.05) (\aleft - 2, \y - 2.2) (\aleft - 3, \y -2.3)};
\draw [->, >=stealth, thick,shorten >=2pt] plot [smooth] coordinates {(\aleft - 3, \y -4) (\aleft - 2, \y - 3.7) (\aleft, \y-2.3) };

%%% Reduce
\path[->]
(-\x - 3.5, 2.2)  edge node [label, left] {\footnotesize{$\bar{x}$}} (-\x - 3.5, 1.4);
\path[->]	
(-\x - 3.5, -0.2) [dashed] edge node [label, left] {} (-\x - 3.5, 0.6)
(-\x - 3, 0.6) [dashed] edge node [label, right] {\footnotesize{\MQ($x'$)}} (-\x - 3, -0.2);

%%% MQ
\draw [->, >=stealth, thick,shorten >=2pt] plot [smooth] coordinates {(\aleft, -0.7) (\aleft -1, - 0.65) (\aleft - 2,  - 0.45) (\aleft - 3, -0.4)};
\draw [->, >=stealth, thick,shorten >=2pt] plot [smooth] coordinates {(\aleft - 3, -0.8)(\aleft - 2,  - 0.8)(\aleft -1, - 0.95) (\aleft, -1)  };


\end{tikzpicture}

==> tikz/soundness-counterexample.tex <==
\begin{tikzpicture}
\definecolor{orange}{HTML}{ec9a29}


	
	\node [comp, accepting, initial] (q0) {$q_0$};
	\node [comp, right = 5em of q0](q1) {$q_{1}$};
	
	\path[->]
	(q0) edge [loop above] node [label, above] {$(a,a)\vee(\neg a, \neg a) \vee (\neg a, a)$} (q0)
	(q0) edge node [label, below] {$(a,\neg a) $} (q1)
	(q1) edge [loop above] node [label, above] {$\top$} (q1);
	

	
\end{tikzpicture}
